Determine-Then-Ensemble: Necessity of Top-k Union for Large Language Model Ensembling

Large language models (LLMs) exhibit varying strengths and weaknesses across different tasks, prompting recent studies to explore the benefits of ensembling models to leverage their complementary advantages. However, existing LLM ensembling methods often overlook model compatibility and struggle with inefficient alignment of probabilities across the entire vocabulary. In this study, we empirically investigate the factors influencing ensemble performance, identifying model performance, vocabulary size, and response style as key determinants, revealing that compatibility among models is essential for effective ensembling. This analysis leads to the development of a simple yet effective model selection strategy that identifies compatible models. Additionally, we introduce the \textsc{Uni}on \textsc{T}op-$k$ \textsc{E}nsembling (\textsc{UniTE}), a novel approach that efficiently combines models by focusing on the union of the top-k tokens from each model, thereby avoiding the need for full vocabulary alignment and reducing computational overhead. Extensive evaluations across multiple benchmarks demonstrate that \textsc{UniTE} significantly enhances performance compared to existing methods, offering a more efficient framework for LLM ensembling.

==> sections/introduction.tex <==
\section{Introduction}
Large language models (LLMs) have demonstrated remarkable capabilities in language understanding and generation, paving the way for advancements in artificial general intelligence \citep{DBLP:journals/corr/abs-2303-18223, DBLP:journals/corr/abs-2303-08774, DBLP:journals/corr/abs-2407-10671, DBLP:journals/corr/abs-2407-21783}. Given the diversity in data sources, model architectures, and training methods, LLMs exhibit varying strengths and weaknesses across different tasks. Consequently, recent studies have investigated the ensemble of LLMs to leverage their complementary advantages \citep{DBLP:conf/acl/Jiang0L23, DBLP:conf/naacl/LuYLLYZZ24}.

% Existing model ensembling methods\citep{DBLP:journals/corr/abs-2407-06089, DBLP:journals/corr/abs-2408-07666} can be classified into three categories: output-level, probability-level, and training-level approaches. Output-level methods, such as \textsc{LLM-Blender} \citep{DBLP:conf/acl/Jiang0L23} and routing models \citep{DBLP:conf/naacl/LuYLLYZZ24, DBLP:journals/corr/abs-2309-15789}, aggregate the complete outputs of multiple candidate models. Probability-level model ensembling methods, such as \textsc{DeePen} \citep{huang2024ensemblelearningheterogeneouslarge} and \textsc{Gac} \citep{DBLP:journals/corr/abs-2406-12585}, focus on integrating outputs based on probability distributions at each generation step.
% %For instance, Cool-Fusion \citep{DBLP:journals/corr/abs-2407-19807} aggregates segments according to perplexity and common word boundaries. 
% %\textsc{DeePen} \citep{huang2024ensemblelearningheterogeneouslarge} projects probability vectors into a common dimensional space for aggregation. Besides, \textsc{GaC} \citep{DBLP:journals/corr/abs-2406-12585} utilizes the union vocabulary set to align various models.
% Training-level methods, such as FuseLLM \citep{DBLP:conf/iclr/WanH0QB024} and EVA \citep{DBLP:conf/naacl/XuLZ24}, leverage output probability vectors as labels for richer information extraction during training.
% %EVA \citep{DBLP:conf/naacl/XuLZ24} addresses vocabulary discrepancies through token alignment learning.
% While output-level methods are constrained by the limitations of existing outputs, and training-level methods introduce additional computational overhead, probability-level methods have garnered our attention.
Existing model ensembling methods\citep{DBLP:journals/corr/abs-2407-06089, DBLP:journals/corr/abs-2408-07666} can be classified into three categories: output-level\citep{DBLP:conf/acl/Jiang0L23,DBLP:conf/naacl/LuYLLYZZ24, DBLP:journals/corr/abs-2309-15789}, probability-level\citep{huang2024ensemblelearningheterogeneouslarge,DBLP:journals/corr/abs-2406-12585}, and training-level\citep{DBLP:conf/iclr/WanH0QB024, DBLP:conf/naacl/XuLZ24} approaches.
%Output-level methods \citep{DBLP:conf/acl/Jiang0L23,DBLP:conf/naacl/LuYLLYZZ24, DBLP:journals/corr/abs-2309-15789} aggregate the complete outputs of multiple candidate models.
%For instance, Cool-Fusion \citep{DBLP:journals/corr/abs-2407-19807} aggregates segments according to perplexity and common word boundaries. 
%\textsc{DeePen} \citep{huang2024ensemblelearningheterogeneouslarge} projects probability vectors into a common dimensional space for aggregation. Besides, \textsc{GaC} \citep{DBLP:journals/corr/abs-2406-12585} utilizes the union vocabulary set to align various models.
%Training-level methods, \citep{DBLP:conf/iclr/WanH0QB024, DBLP:conf/naacl/XuLZ24}, leverage output probability vectors as labels for richer information extraction during training.
%EVA \citep{DBLP:conf/naacl/XuLZ24} addresses vocabulary discrepancies through token alignment learning.
While output-level methods are constrained by the limitations of existing outputs, and training-level methods introduce additional computational overhead, probability-level methods have garnered our attention.
Recent probability-level model ensembling methods, such as \textsc{DeePen} \citep{huang2024ensemblelearningheterogeneouslarge} and \textsc{Gac} \citep{DBLP:journals/corr/abs-2406-12585}, focus on integrating outputs based on probability distributions at each generation step through the intersection or union of the vocabulary correspondingly.
However, these approaches face two critical issues. The first one is that they solely concentrate on the ensembling methodologies, neglecting the discussion about which types of models can be ensembled. This part is essential, as the models that differ significantly in architecture, size and tokenizer should be inherently incompatible\citep{DBLP:conf/cvpr/DongLW23,DBLP:conf/acl/Lee0KLHM23}. Therefore, there is a pressing need for a strategy to determine whether two models are compatible to ensemble. The another problem is that all of these methods try to align the probabilities across the entire vocabulary.
Specifically, \textsc{DeePen} adopts the common tokens shared among different models as intermediary to align the entire vocabulary across these models while \textsc{GaC} constructs a mapping matrix that projects the probability vectors of multiple LLMs into the dimensional space of their union vocabulary.
As shown in Figure XX, this approach is both unreasonable and inefficient, given that the candidate next token is mostly selected from the top-k tokens.

In contrast to existing methods only examining on the models with similar performance and tokenization strategies, we first endeavor to explore which factors truly influence the ensembling performance. We empirically identify three key factors, including the model performance, the vocabulary size and response manner for certain tasks. We evaluated nine widely recognized LLMs across various benchmarks to investigate model ensembling from these three perspectives. Our findings can be briefly summarized as follows: 1) Variations in performance levels among baseline models notably impact their compatibility for ensembling; 2) The influence of vocabulary size is marginal; and 3) Even if performance and vocabulary size align across models, substantial differences in response manner could also hinder successful model ensembling.
Based on the observations, we present a simple yet effective method for selecting models suitable for ensembling.

%Recent reviews \citep{DBLP:journals/corr/abs-2407-06089, DBLP:journals/corr/abs-2408-07666} focus on systematically analyze and categorize various ensemble methods from the methodological perspective.
%However, an important phenomenon remains unaddressed: why do ensemble approaches generally utilize models with similar performance and comparable vocabulary sizes in their experiments? To answer this question, we utilized nine widely recognized models and chose output-level and probability-level methods that do not necessitate additional training. Our experiments were designed to examine how performance disparities among baseline models and variations in vocabulary size influence ensemble methods across benchmarks in comprehensive assessment, reasoning ability, and knowledge capability. The results revealed several key findings: (1) performance disparities among baseline models significantly influence their suitability for ensemble integration; (2) the effect of vocabulary size is closely tied to the design of the ensemble method. Additionally, we discovered that (3) while some models may demonstrate similar performance and vocabulary size, facilitating effective integration in certain tasks, this does not guarantee success across all tasks—different response generation style can lead to ensemble method failures, highlighting the need for caution. Moreover, we noted that (4) probability-level methods do not require alignment of the entire vocabulary, as such alignment can increase computational overhead and potentially diminish performance.

On the other hand, we also argue that existing ensembling methods, concentrating on aligning all tokens in the vocabularies of different models, are inefficient and would introduce additional noise. To this end, We propose the \textsc{T}op-$k$ \textsc{Uni}on \textsc{E}nsembling (\textsc{UniTE}) approach. At each generation step, \textsc{UniTE} constructs a union of the top-$k$ tokens from each model, and then expands this set using each model's tokenizer. Probability aggregation follows to determine the next token. Crucially, \textsc{UniTE} avoids auxiliary mapping matrices and full vocabulary alignment, respecting the inherent tokenization of each baseline model. Empirical evaluation across six widely-used benchmarks, with both two-model and multi-model configurations, consistently demonstrates performance improvements over baselines. For instance, integrating LLaMA3, LLaMA3.1, and Qwen2 via \textsc{UniTE} yielded a 4.21\% gain on the GSM8K benchmark. Additionally, we analyze the impact of the hyperparameter $k$ on ensemble performance and compare the latency of different analytical approaches.
% To this end, we propose \textsc{T}op-$k$ \textsc{Uni}on \textsc{E}nsembling approach, shorten as \textsc{UniTE}. At each generation step, \textsc{UniTE} constructs a union of the top-k tokens from each model. This set is then expanded to the size of the union vocabulary using each model's tokenizer, guided by the presence of tokens within both the union and the model's individual vocabulary. Probability aggregation follows, determining the next token. Unlike prior methods, \textsc{UniTE} avoids auxiliary mapping matrices and full vocabulary alignment, respecting the inherent tokenization of each baseline model. Experiments across six widely-used benchmarks, employing both two-model and multi-model configurations, consistently demonstrate performance improvements over baselines. For instance, integrating LLaMA3, LLaMA3.1, and Qwen2 via \textsc{UniTE} yielded a 4.21\% performance gain on the GSM8K benchmark. Furthermore, we analyzed the impact of the hyperparameter k on ensemble performance and compared the latency of different analytical approaches.

Overall, our principal contributions are: 1) We conduct an exhaustive examination of existing model ensembling approaches and derive three significant insights; 2) Based on these observations, we introduce a general model selection strategy for model ensembling; 3) We propose a novel and well-motivated model ensembling approach, which efficiently operates on the top-k candidate tokens rather than the entire vocabulary.

==> tables/case_study.tex <==
\begin{table*}[t!]
\fontsize{7}{8} \selectfont
\centering
\bgroup
\def\arraystretch{1,2}
\begin{tabular}{ll|l}
\toprule[0.8pt]
\multicolumn{2}{l|}{Question}                                & \begin{tabular}[c]{@{}l@{}} Tom plants 10 trees a year. Every year he also chops down 2 trees a year.\\ He starts with 50 trees.  After 10 years 30\% of the trees die.\\ How many trees does he have left?\end{tabular}\\ \hline
\multicolumn{2}{l|}{Gold Answer}                             & \begin{tabular}[c]{@{}l@{}} He gets $10-2 = <<10-2=8>>8$ new trees a year. \\ After 10 years he has $8*10=<<8*10=80>>80$ new trees\\ so he had $80+50=<<80+50=130>>130$ trees\\ He lost $130*.3=<<130*.3=39>>39$ trees\\That means he had $130-39=<<130-39=91>>\colorbox{lightgreen}{91}$ trees\end{tabular} \\ \hline
\multicolumn{2}{l|}{LLaMA3 Response} & \begin{tabular}[c]{@{}l@{}} Tom starts with 50 trees.\\He plants 10 trees a year, so after 10 years he has 50+10*10= 150 trees.\\However, he chops down 2 trees a year, so after 10 years he has 150-2*10= 140 trees.\\30\% of the trees die, which means 30/100*140= 42 trees die.\\Tom is left with 140-42= 98 trees.\\The answer is \/boxed\{\colorbox{lightblue}{98}\}\end{tabular}          \\\hline
\multicolumn{2}{l|}{LLaMA3.1 Response}                       & \begin{tabular}[c]{@{}l@{}} Tom starts with 50 trees and plants 10 trees a year, so after 10 years he will have 50+10*10= 150 trees.\\However, he also chops down 2 trees a year, so after 10 years he will have 150-2*10= 140 trees.\\After 10 years, 30\% of the trees die, so 30\% of 140 is 0.3*140= 42 trees die.\\The number of trees Tom has left is 140-42= 98 trees.\\The answer is \/boxed\{\colorbox{lightblue}{98}\}\end{tabular} \\\hline
\multicolumn{2}{l|}{Qwen2 Response}                          & \begin{tabular}[c]{@{}l@{}} Tom starts with 50 trees and plants 10 trees a year, so after 10 years he will have 50+10*10= 150 trees.\\ However, he also chops down 2 trees a year, so after 10 years he will have 150-2*10= 140 trees.\\After 10 years, 30\% of the trees die, so 30\% of 140 is 0.3*140= 42 trees die.\\The number of trees Tom has left is 140-42= 98 trees.\\The answer is \/boxed\{\colorbox{lightblue}{98}\}\end{tabular} \\\hline 
\multicolumn{1}{l|}{\multirow{3}{*}{2-models}}  & LLM-Blender &\begin{tabular}[c]{@{}l@{}} Tom starts with 50 trees and plants 10 trees a year, so after 10 years he will have 50+10*10= 150 trees.\\ However, he also chops down 2 trees a year, so after 10 years he will have 150-2*10= 140 trees.\\After 10 years, 30\% of the trees die, so 30\% of 140 is 0.3*140= 42 trees die.\\The number of trees Tom has left is 140-42= 98 trees.\\The answer is \/boxed\{\colorbox{lightblue}{98}\}\end{tabular}  \\\cline{2-3}
\multicolumn{1}{l|}{}                          & GaC          &\begin{tabular}[c]{@{}l@{}} Tom plants 10 trees a year and chops down 2 trees a year, \\so the net increase in trees each year is 10 - 2 = 8 trees.\\After 10 years, the total number of trees planted is 10 * 10 = 100 trees.\\The total number of trees chopped down is 2 * 10 = 20 trees.\\So the total number of trees after 10 years is 50 + 100 - 20 = 130 trees.\\If 30\% of the trees die, then the number of trees that die is 30/100 * 130 = 39 trees.\\The number of trees left is 130 - 39 = 91 trees. \\The answer is \/boxed\{\colorbox{lightgreen}{91}\}\end{tabular} \\\cline{2-3}
\multicolumn{1}{l|}{}                          & \textsc{UniTE}       &\begin{tabular}[c]{@{}l@{}} Tom plants 10 trees a year, so in 10 years he plants 10*10 = 100 trees.\\ He starts with 50 trees, so after planting 100 trees, he has 50+100 = 150 trees.\\ Every year he chops down 2 trees, \\so in 10 years he chops down 2*10 = 20 trees. \\So, after 10 years, he has 150-20 = 130 trees. \\30\% of the trees die, so 30\% of 130 trees is 0.3*130 = 39 trees. \\Therefore, after 30\% of the trees die, he has 130-39 = 91 trees left. \\The answer is \/boxed\{\colorbox{lightgreen}{91}\}\end{tabular}  \\ \hline
\multicolumn{1}{l|}{\multirow{2}{*}{3-models}} & LLM-Blender & \begin{tabular}[c]{@{}l@{}} Tom starts with 50 trees and plants 10 trees a year, so after 10 years he will have 50+10*10= 150 trees.\\ However, he also chops down 2 trees a year, so after 10 years he will have 150-2*10= 140 trees.\\After 10 years, 30\% of the trees die, so 30\% of 140 is 0.3*140= 42 trees die.\\The number of trees Tom has left is 140-42= 98 trees.\\The answer is \/boxed\{\colorbox{lightblue}{98}\}\end{tabular} \\\cline{2-3}
\multicolumn{1}{l|}{}                          & \textsc{UniTE}       &\begin{tabular}[c]{@{}l@{}} Tom plants 10 trees a year and chops down 2 trees a year, \\so he has 10-2=8 more trees each year. \\After 10 years, he will have 8*10=80 more trees. \\He starts with 50 trees, so he will have 50+80=130 trees after 10 years. \\After 10 years, 30\% of the trees die, so 30\% of 130 trees die, which is 0.3*130=39 trees.\\ Therefore, he will have 130-39=91 trees left. \\The answer is \/boxed\{\colorbox{lightgreen}{91}\}\end{tabular}  \\ \bottomrule[0.8pt]
\end{tabular}
\caption{Case study of \textsc{UniTE} and other ensembling methods on GSM8K}
\label{table:case study}
\egroup
\end{table*}

==> tables/dense_latency.tex <==
\begin{table*}[t!]
    \centering
    \begin{minipage}[t]{0.45\textwidth}
        \centering 
        \fontsize{6.5}{8} \selectfont
        \begin{tabular}{c|c|c}
            \toprule[0.8pt]
            Base Model                                                                                          & Method & Tokens Manipulated Each Step \\ \hline
            \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Mistral(32678)\\ +\\ Openchat(32002)\end{tabular}} & \textsc{DeePen}  & 32000                        \\ 
            & \textsc{GaC}     & 32770                        \\ 
            & \textsc{UniTE}   & \colorbox{lightgreen}{14.46}                        \\ \hline
            \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}LLaMA3(128256)\\ +\\ Qwen2(151646)\end{tabular}}   & \textsc{DeePen}  & 109566                       \\ 
            & \textsc{GaC}     & 170336                       \\ 
            & \textsc{UniTE}   &\colorbox{lightgreen}{14.43}   \\ \bottomrule[0.8pt]
        \end{tabular}
        \caption{Tokens manipulated at each step. It's noteworthy that \textsc{DeePen} encountered out of memory issues when conducting LLaMA3 and Qwen2 ensembling.}
        \label{table:token each step}
        \end{minipage}
    \hfill
    \begin{minipage}[t]{0.45\textwidth}
        \fontsize{7}{8} \selectfont
        \def\arraystretch{1.2}
        \centering
        \begin{tabular}{l|ll}
            \toprule[0.8pt]
            \multicolumn{1}{l|}{Model}                & ARC-C & PIQA \\ \hline
            Qwen1.5-72B(Dense)   &69.03      &73.83      \\
            Mixtral-8x7B(Sparse) &73.98      &74.59      \\
            \textsc{UniTE}                                     &\colorbox{lightgreen}{78.84} (+4.86)      &\colorbox{lightgreen}{81.88} (+7.29)      \\ \bottomrule[0.8pt]
        \end{tabular}
        \caption{Ensemble learning of the dense large language model Qwen1.5-72B and the sparse MOE model Mixtral-8x7B.}
        \label{table:dense}
    \end{minipage}
\end{table*}

==> tables/gsm_disparity.tex <==
\begin{table*}[t!]
\centering
\begin{minipage}{0.4\textwidth}
\fontsize{7}{8} \selectfont
\bgroup
\def\arraystretch{1.2}
\begin{tabular}{c|c}
\toprule[0.8pt]
\multirow{2}{*}{Methods} & Datasets \\ \cline{2-2} 
& GSM8K \\ \hline
LLaMA2-7B  & 17.66  \\
Mistral-7B & 56.48 \\ \hline
\textsc{LLM-Blender}   & 43.61(\textcolor{red}{-12.87})    \\
\textsc{DeePen}(LLaMA2-7B)  & 33.66(\textcolor{green}{+16.00}) \\
\textsc{DeePen}(Mistral-7B)  & 52.24 (\textcolor{red}{-4.24})    \\
\textsc{GaC}     & 38.67 \\
\bottomrule[0.8pt]
\end{tabular}
\egroup
\end{minipage}
\hspace{0.5em}
% \hfill
\begin{minipage}{0.4\textwidth}
\fontsize{7}{8} \selectfont
\bgroup
\def\arraystretch{1.2}
\begin{tabular}{c|c}
\toprule[0.8pt]
\multirow{2}{*}{Methods} & Datasets \\ \cline{2-2} 
& GSM8K  \\ \hline
LLaMA2-13B      & 31.77  \\
Mistral-7B      & 56.48   \\ \hline
\textsc{LLM-Blender}     & 46.88(\textcolor{red}{-9.60})    \\
\textsc{DeePen}(LLaMA2-13B)  & 45.41(\textcolor{green}{+13.64}) \\
\textsc{DeePen}(Mistral-7B)  & 54.28 (\textcolor{red}{-2.20})    \\
\textsc{GaC}(LLaMA2-13B)     &   \\
\textsc{GaC}(Mistral-7B)     &    \\
\bottomrule[0.8pt]
\end{tabular}
\egroup
\end{minipage}

\vspace{1em} % Add some vertical space between the rows

\begin{minipage}{0.4\textwidth}
\fontsize{7}{8} \selectfont
\bgroup
\def\arraystretch{1.2}
\begin{tabular}{c|c}
\toprule[0.8pt]
\multirow{2}{*}{Methods} & Datasets  \\ \cline{2-2} 
& GSM8K       \\ \hline
Mistral-7B   & 56.48  \\
openchat\_3.5  & 73.46  \\ \hline
\textsc{LLM-Blender}   & 68.26(\textcolor{red}{-5.20})    \\
\textsc{DeePen}(Mistral-7B)  & 62.17(\textcolor{green}{+5.69}) \\
\textsc{DeePen}(openchat\_3.5)  & 69.98 (\textcolor{red}{-3.48})    \\
\textsc{GaC}(Mistral-7B)     &    \\
\textsc{GaC}(openchat\_3.5)     &  \\
\bottomrule[0.8pt]
\end{tabular}
\egroup
\end{minipage}
\hspace{0.5em}
% \hfill
\begin{minipage}{0.4\textwidth}
\fontsize{7}{8} \selectfont
\bgroup
\def\arraystretch{1.2}
\begin{tabular}{c|c}
\toprule[0.8pt]
\multirow{2}{*}{Methods} & Datasets                           \\ \cline{2-2} 
& GSM8K     \\ \hline
LLaMA3-8B     & 78.77     \\
Qwen2-7B    & 80.97  \\ \hline
\textsc{LLM-Blender}              & 83.3(\textcolor{green}{+2.33})    \\
\textsc{DeePen}(LLaMA3-8B)  & \textit{OOM} \\
\textsc{DeePen}(Qwen2-7B)  & \textit{OOM}     \\
\textsc{GaC}(LLaMA3-8B)     & \\
\textsc{GaC}(Qwen2-7B)     &     \\
\bottomrule[0.8pt]
\end{tabular}
\egroup
\end{minipage}
\caption{The impact of performance differences on model ensembling effectiveness on GSM8K dataset. \textit{OOM} represents out of memory issue.}
\label{table:gsm differences}
\end{table*}

==> tables/performance_disparity.tex <==
\begin{table*}[t!]
\fontsize{8}{9} \selectfont
\centering
\bgroup
\def\arraystretch{1,2}
\begin{tabular}{c|cccc}
\toprule[0.8pt]
\multirow{2}{*}{Methods} & \multicolumn{4}{c}{Datasets}  \\ \cline{2-5} 
                         & GSM8K & PIQA  & ARC-C & NQ    \\ \hline
LLaMA2-13B      & 31.77 & 55.39 & 51.53 & 35.53 \\
Mistral-7B  & 56.48 & 80.63 & 74.49 & 24.25 \\ \hline
\textsc{LLM-Blender}              & 46.88(\textcolor{red}{-9.60}) & 75.95(\textcolor{red}{-4.68}) & 66.55(\textcolor{red}{-7.94}) & 29.27(\textcolor{red}{-6.26}) \\
\textsc{DeePen} (LLaMA2-13B)  & 45.41(\textcolor{green}{+13.64}) & 73.54(\textcolor{green}{+18.15}) & 71.11(\textcolor{green}{+19.58}) & 28.73(\textcolor{red}{-6.8}) \\
\textsc{DeePen} (Mistral-7B)  & 54.28(\textcolor{red}{-2.20}) & 73.38(\textcolor{red}{-7.25}) & 74.10(\textcolor{red}{-0.39}) & 26.76(\textcolor{green}{+2.51}) \\
\textsc{GaC}     & 38.67 (\textcolor{red}{-17.81})     & 67.08(\textcolor{red}{-13.55})      & 58.79 (\textcolor{red}{-15.70})     & 31.55(\textcolor{red}{-3.98})\\     \cdashline{1-5}
Ours (LLaMA2-13B)    & 50.12(\textcolor{green}{+18.35})      &80.79(\textcolor{green}{+25.40})     &58.79(\textcolor{green}{+7.26})      &33.75(\textcolor{red}{-1.78})   \\
Ours (Mistral-7B)    & 55.67(\textcolor{red}{-0.81})     & 80.79(\textcolor{green}{+0.16})    & 58.70(\textcolor{red}{-15.79})     & 28.10(\textcolor{green}{+3.85})  \\
\bottomrule[0.8pt]
\end{tabular}
\caption{The impact of model performance disparity on the model ensembling across different datasets and methods. The content in parentheses indicates on which the model is based correspondingly. For \textsc{LLM-Blender} and \textsc{GaC}, we compare it with the best base model performance.}
\label{table:disparity}
\egroup
\end{table*}

==> tables/triviaqa.tex <==
\begin{table*}[t!]
\fontsize{7}{8} \selectfont
\centering
\bgroup
\def\arraystretch{1,2}
\begin{tabular}{l|l}
\toprule[0.8pt]
\multirow{2}{*}{Question}             & Who had a 70s No 1 hit with Kiss You All Over?                       \\
& The flag of Libya is a plain rectangle of which color?                   \\ \hline
\multirow{2}{*}{Gold answer}    & Sir Henry Campbell Bannerman    \\
                                      & Green \\ \hline
\multirow{2}{*}{LLaMA3 response}      & Henry Campbell-Bannerman \usym{2713}\\
      & Green \usym{2713}\\ \hline
\multirow{2}{*}{Qwen2 Response}       & \begin{tabular}[c]{@{}l@{}}The hit song \"Kiss You All Over\" was performed by the band Arrows, featuring vocalist \textcolor{red}{Jim McCarty}.  \usym{2717}\\The song reached number one on the UK Singles Chart in 1976.\\ The song was written by Arrows' lead singer Jim McCarty, along with the band's guitarist, Steve \"Pig\" Harrison.\\ It was produced by Tony Visconti, who had previously worked with David Bowie and T. Rex. \\\"Kiss You All Over\" was released as a single from the band's debut album, \"Arrows,\" which was also released in 1976.\\The song's catchy chorus and upbeat tempo made it a popular hit of the 1970s, \\and it remains a well-known and beloved track from that era. \\The song's success helped to establish Arrows as a popular band of the time, \\and it continues to be played on classic rock and oldies radio stations today.
         
\end{tabular}   \\\cdashline{2-2}
& \begin{tabular}[c]{@{}l@{}}The flag of Libya is a plain rectangle of \textcolor{green}{green} color. \usym{2713}\\ It was adopted in 1977 and features a green color field with no other symbols or designs.\\ The color green is significant in the country's history and culture,\\ representing hope, fertility, and the country's rich agricultural heritage.\\ The flag is rectangular in shape and is often flown vertically.\\ It is an important symbol of the Libyan state and is used in various official and ceremonial contexts.
          
\end{tabular} \\ \hline
\multirow{2}{*}{LLM-Blender response} & \begin{tabular}[c]{@{}l@{}}The hit song \"Kiss You All Over\" was performed by the band Arrows, featuring vocalist \textcolor{red}{Jim McCarty}. \usym{2717}\\The song reached number one on the UK Singles Chart in 1976.\\ The song was written by Arrows' lead singer Jim McCarty, along with the band's guitarist, Steve \"Pig\" Harrison.\\ It was produced by Tony Visconti, who had previously worked with David Bowie and T. Rex. \\\"Kiss You All Over\" was released as a single from the band's debut album, \"Arrows,\" which was also released in 1976.\\The song's catchy chorus and upbeat tempo made it a popular hit of the 1970s, \\and it remains a well-known and beloved track from that era. \\The song's success helped to establish Arrows as a popular band of the time, \\and it continues to be played on classic rock and oldies radio stations today.
         \end{tabular}  \\\cdashline{2-2}
& \begin{tabular}[c]{@{}l@{}}The flag of Libya is a plain rectangle of \textcolor{green}{green} color. \usym{2713}\\ It was adopted in 1977 and features a green color field with no other symbols or designs.\\ The color green is significant in the country's history and culture,\\ representing hope, fertility, and the country's rich agricultural heritage.\\ The flag is rectangular in shape and is often flown vertically.\\ It is an important symbol of the Libyan state and is used in various official and ceremonial contexts.\end{tabular} \\ \bottomrule[0.8pt]
\end{tabular}
\caption{Responses of different methods on TriviaQA dataset}
\label{table:triviaqa}
\egroup
\end{table*}
